GAM-RAG: Gain-Adaptive Memory for Evolving Retrieval in Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) grounds large language models with external evidence, but many implementations rely on pre-built indices that remain static after construction. Related queries therefore repeat similar multi-hop traversal, increasing latency and compute. Motivated by schema-based learning in cognitive neuroscience, we propose GAM-RAG, a training-free framework that accumulates retrieval experience from recurring or related queries and updates retrieval memory over time. GAM-RAG builds a lightweight, relation-free hierarchical index whose links capture potential co-occurrence rather than fixed semantic relations. During inference, successful retrieval episodes provide sentence-level feedback, updating sentence memories so evidence useful for similar reasoning types becomes easier to activate later. To balance stability and adaptability under noisy feedback, we introduce an uncertainty-aware, Kalman-inspired gain rule that jointly updates memory states and perplexity-based uncertainty estimates. It applies fast updates for reliable novel signals and conservative refinement for stable or noisy memories. We provide a theoretical analysis of the update dynamics, and empirically show that GAM-RAG improves average performance by 3.95% over the strongest baseline and by 8.19% with 5-turn memory, while reducing inference cost by 61%. Our code and datasets are available at: https://anonymous.4open.science/r/GAM_RAG-2EF6.

==> 1_Introduction.tex <==
% outline
% draft
Retrieval-Augmented Generation (RAG) has become a key paradigm for augmenting LLMs with external knowledge bases~\cite{zhang2025surveygraphretrievalaugmentedgeneration,sharma2025retrievalaugmentedgenerationcomprehensivesurvey}. 
However, conventional vector-based RAG lacks the ability to capture long-range dependencies and to reliably support multi-hop reasoning~\cite{peng2024graphretrievalaugmentedgenerationsurvey,procko2024graph}. 
To address this, hybrid RAG methods build structured indices to explicitly model document connectivity. 
% GraphRAG~\cite{han2024retrieval} constructs a graph-structured index over the corpus to support coarse-to-fine retrieval. 
\textcolor{blue}{As a representative hybrid approach, GraphRAG~\cite{han2024retrieval} builds a corpus-level graph index and performs coarse-to-fine retrieval.}
More recently, GFM-RAG~\cite{luo2025gfmraggraphfoundationmodel} and HippoRAG2~\cite{gutierrez2025rag} further integrate graph propagation via graph neural networks and personalized PageRank, leading to strong performance on on multi-hop reasoning tasks. 


\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{Fig/fig1.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Motivation. (a) Without memory storage, similar queries still require same iterations to the answer. (b) Without memory update, replaying noisy traces can mislead reasoning.}
\label{fig1}
\end{figure} 

Despite their strong performance, KG-based approaches face notable cost and robustness challenges~\cite{hu2025remindraglowcostllmguidedknowledge}. 
% First, they typically rely on LLM-driven KG construction, yet recent studies show that explicit relation extraction in complex contexts can incur substantial overhead and may lose critical semantics during structuring~\cite{zhu2025knowledgegraphguidedretrievalaugmented}. 
\textcolor{blue}{First, they typically rely on LLM-driven KG construction, which makes relation extraction in complex contexts expensive; moreover, the structuring process can drop subtle but important semantics~\cite{zhu2025knowledgegraphguidedretrievalaugmented}. }
% Second, at inference time, traversal over structured knowledge is largely guided by the LLMs' semantic understanding and decision-making~\cite{kashmira-etal-2025-tobugraph}, but lacks a memory mechanism to retain experience and learn from past retrieval outcomes. 
\textcolor{blue}{Second, at inference time,  traversal is largely guided by the LLM’s semantic judgments~\cite{kashmira-etal-2025-tobugraph}. However, current traversal policies rarely leverage historical success or failure signals and lack an explicit memory to learn from past retrieval outcomes. }
% As a result, retrieval quality depends heavily on the underlying LLM, leading to largely fixed reasoning cost and a performance ceiling. 【这句话删掉了，我觉得和前面的逻辑不连贯，】
% As illustrated in fig~\ref{fig1}(a), KG-based methods still runs the same full retrieval-and-reasoning procedure even for previously solved, similar queries; and it has limited feedback to learn from previously failed queries once retrieval goes astray.
\textcolor{blue}{As illustrated in fig~\ref{fig1}(a), KG-based methods still runs the same full retrieval-and-reasoning procedure even for previously solved, similar queries; and it has limited feedback to learn from previously failed queries once retrieval goes astray.}

% Recent efforts have begun to store  experience by logging past successful episodes and retrieving them as additional in-context guidance, such as through case-based prompt augmentation~\cite{wiratunga2024cbrragcasebasedreasoningretrieval} or by explicitly storing and recalling intermediate thought traces to steer future reasoning~\cite{feng2024thoughtretriever}.
\textcolor{blue}{To mitigate this issue, recent work has explored experience reuse by logging successful episodes and retrieving them to provide in-context guidance. 
Specifically, prior studies augment prompts with similar solved cases~\cite{wiratunga2024cbrragcasebasedreasoningretrieval} or store and recall intermediate reasoning traces to steer future reasoning~\cite{feng2024thoughtretriever}.}
However, these approaches typically treat experience as discrete textual samples that are re-injected into the prompt, which can accumulate substantial context overhead as the number and length of traces grow~\cite{terranova2025evaluatinglongtermmemorylongcontext}.
Moreover, they often lack the mechanism to quantify and adapt the reliability of each stored experience, making it non-trivial to robustly match, weight, and update memories when retrieval outcomes are uncertain or partially correct~\cite{wang2025retrievalaugmentedgenerationconflictingevidence}. As shown in fig~\ref{fig1}(b), when recalled memory is unreliable, injecting them can introduce substantial noise that distracts retrieval and reasoning, ultimately leading to incorrect answers.

To this end, we propose \textbf{GAM-RAG}, a gain-adaptive memory framework that continuously updates experiential knowledge without additional training. 
GAM-RAG addresses the above limitations through three key designs: 
(i) a \emph{relation-free} hierarchical graph index that connects entities, sentences, and passages, avoiding the cost and semantic loss of explicit relation extraction; 
(ii) a \emph{memory-driven} iterative search mechanism that leverages sentence-level memories to more precisely match evidence in multi-hop traversal, while reaching the target evidence in fewer iterations; and 
(iii) an \emph{uncertainty-aware} memory update mechanism that jointly updates memory states and perplexities, suppressing noisy or unreliable experiences and preventing low-quality memories from degrading retrieval.

Specifically, GAM-RAG first builds a relation-free hierarchical index that links entities, sentences, and passages via co-occurrence and containment, and initializes sentence-level task and time memories together with their perplexities. During inference, it performs memory-guided iterative retrieval: activated entities propagate to sentences and passages, while the stored memories steer traversal toward evidence that is both semantically relevant and temporally consistent. After each iteration, GAM-RAG updates memory states and their perplexities with an uncertainty-aware gain mechanism, allowing reliable experiences to be absorbed quickly while preventing noisy or unreliable memories from introducing distraction. To evaluate GAM-RAG, we conduct experiments on multi-hop and time-sensitive QA benchmarks, measuring both retrieval quality and inference efficiency, and show that GAM-RAG consistently outperforms strong hybrid-RAG baselines with lower reasoning overhead. Overall, our contributions are threefold.
\begin{itemize}
\item We introduce GAM-RAG, a training-free gain-adaptive memory framework that learns retrieval experience and reuses it to multi-hop evidence discovery.
\item We develop an uncertainty-aware Kalman-inspired update rule that jointly updates memory states and perplexities, mitigating noisy or unreliable memories.
\item We validate GAM-RAG both theoretically and empirically across diverse settings, demonstrating consistent gains in retrieval quality and inference efficiency.
\end{itemize}


